Categorizing Comparative Sentences

We tackle the tasks of automatically identifying comparative sentences and categorizing the intended preference (e.g., "Python has better NLP libraries than MATLAB" => (Python, better, MATLAB). To this end, we manually annotate 7,199 sentences for 217 distinct target item pairs from several domains (27% of the sentences contain an oriented comparison in the sense of "better" or "worse"). A gradient boosting model based on pre-trained sentence embeddings reaches an F1 score of 85% in our experimental evaluation. The model can be used to extract comparative sentences for pro/con argumentation in comparative / argument search engines or debating technologies.

==> table-baseline-performance.tex <==

\begin{table}[b]
   \caption{Best results of the classifier-based model as compared to the keyword-based baseline.}
\small
    \vspace*{3mm}
    \centering
    \begin{tabular}{p{1.2cm}cccccc}
    	\toprule[0.02cm]
    	\multicolumn{4}{l}{Unknown position} & \multicolumn{3}{l}{Known position} \\
    	Class & Prec. & Rec. & F1 & Prec. & Rec. & F1 \\\midrule
    	\addlinespace[1ex]	
    	\class{BETTER} & 0.27 & 0.90 & 0.42 & 0.64 & 0.66 & 0.65\\
    	\class{WORSE} & 0.30 & 0.33 & 0.31 & 0.50 & 0.39 & 0.44\\
    	\class{NONE} & 0.95 & 0.37 & 0.53 & 0.89 & 0.90 & 0.90\\
    	Overall & 0.47 & 0.47 & 0.47 & 0.82 & 0.82 & 0.82\\
    	\bottomrule
    \end{tabular}
    \label{tab:baseline_classification}
\end{table}
